Depth Based Semantic Scene Completion with Position Importance Aware Loss

Semantic Scene Completion (SSC) refers to the task of inferring the 3D semantic segmentation of a scene while simultaneously completing the 3D shapes. We propose PALNet, a novel hybrid network for SSC based on single depth. PALNet utilizes a two-stream network to extract both 2D and 3D features from multi-stages using fine-grained depth information to efficiently captures the context, as well as the geometric cues of the scene. Current methods for SSC treat all parts of the scene equally causing unnecessary attention to the interior of objects. To address this problem, we propose Position Aware Loss(PA-Loss) which is position importance aware while training the network. Specifically, PA-Loss considers Local Geometric Anisotropy to determine the importance of different positions within the scene. It is beneficial for recovering key details like the boundaries of objects and the corners of the scene. Comprehensive experiments on two benchmark datasets demonstrate the effectiveness of the proposed method and its superior performance. Models and Video demo can be found at: https://github.com/UniLauX/PALNet.

==> ICAR2020_PALNet/figs/NetworkStructure.tex <==
% 
% 
\begin{figure*}[ht]
\centering
{
\includegraphics[width=\linewidth]{figs/NetworkStructure_v10.pdf}
}
% \vspace{-0.7cm}
\caption{The hybrid network structure of PALNet for semantic scene completion. In depth-stream, 2D CNN is used to process the full resolution depth, the feature maps are projected to 3D space with the 2D-3D projection layer, and followed by 3D convolutions. In voxel-stream, TSDF encoded voxels are sent as input, all convolution operations employed are 3D convolutions. After the two streams of information are aggregated, they are sent to the subsequent network with large receptive field to capture 3D context to predict the complete semantic scene.
We represent the 3D operation in the form of a cuboid in this figure.
Res($c,k,d,s$) is the dilated residual blocks with bottleneck. $c$ is the output channel, $k$ is the kernel size, $d$ is the dilation rate, and $s$ is stride in the convolution. Conv($c,k,d,s$) is the 3D convolutional layer.}
\label{fig:NetworkStructure}
\end{figure*}


==> ICAR2020_PALNet/figs/VoxelPosition.tex <==
% 
% 
\begin{figure*}[ht]
\centering
{
\includegraphics[width=0.95\linewidth]{figs/VoxelPosition_v05.pdf}
}
% \vspace{-0.3cm}
\caption
{Local Geometric Anisotropy: voxels at different positions contain different local geometric information.
(a)-(d) respectively indicate voxels inside the object, voxels on the surface, voxels on the edge, and a voxel on the vertex. For a strip-shaped object, (e),(f) indicate voxels on the edge and a voxel on the vertex.
(g) indicates an isolated voxel.
}
\label{fig:VoxelsPosition}
\end{figure*}


==> ICAR2020_PALNet/figs/curve.tex <==
%
%
%
\begin{figure}[ht]
\centering{\includegraphics[width=1.0\columnwidth]{figs/curve_v2.pdf}}
% \vspace{-1mm}
\caption{
 Training curves of network with different loss functions for scene completion (left) and semantic scene completion (right).
}
\label{fig:curve}
\end{figure}

==> ICAR2020_PALNet/figs/hist_percentage.tex <==
% 
% 
\begin{figure}[ht]
\centering
{
\includegraphics[width=\columnwidth]{figs/hist_percentage_v04.pdf}
}
% \vspace{-8mm}
\caption{
The percentage of voxels with different LGA values in dataset NYU~\cite{silberman2012NYUdataset}. 
More than 84\% of the voxels have $LGA=0$, indicating that most of the voxels are inside the objects, and less than 16\% of the voxels are outside of the objects. Voxels in free space are not taken into account.
}\label{fig:hist}
\end{figure}

==> ICAR2020_PALNet/figs/teaser.tex <==
\begin{figure}[htbp]
\centering{\includegraphics[width=0.95\columnwidth]{figs/teaser_v17.pdf}}
% \vspace{-2mm}
\caption{Semantic Scene Completion: Based on input depth or its corresponding 3D voxel volume, the goal of SSC is to simultaneously complete the partial 3D shapes and predict the dense semantic labels of both observed and unobserved parts in the view frustum.} 
% \vspace{-5mm}
\label{fig:teaser}
\end{figure}

==> ICAR2020_PALNet/figs/vizResults.tex <==
%
%
\begin{figure*}[htbp]
\centering{\includegraphics[width=0.8\linewidth]{figs/vizResults_v9.pdf}}
% \vspace{-2mm}
\caption{For a scene shown in (a), Semantic Scene Completion (SSC) takes (b) depth image as input and output dense 3D semantic volume. (c) gives the ground truth. (d) and (e) are the predictions of the proposed PALNet and SSCNet~\cite{song2017_SSCNet}.
}
% \vspace{-2mm}
\label{fig:vizResults}
\end{figure*}

==> ICAR2020_PALNet/tabs/AS_Accuracy_Different_Loss-Ours.tex <==
\begin{table}[tb]
\caption{Results of PALNet trained with various loss functions.
}
% \vspace{-1mm}
\centering
\begin{tabular}{l|lll|l}
\hline
Loss function & \multicolumn{1}{c}{Precision} & \multicolumn{1}{c}{Recall} & \multicolumn{1}{c|}{IoU} & \multicolumn{1}{c}{mIoU} \\ \hline
WCE Loss    & 79.4               & {\bfseries 95.9}   & 79.9            & 46.3                  \\
Dice Loss   & {\bfseries 88.2}   & 83.3             & 78.64             & 45.3                  \\
Focal Loss   & 85.6               & 91.8            & 79.3              & 46.1                  \\
PA-Loss   & 87.2                  & 91.7            & {\bfseries 80.8}  & {\bfseries 46.6 }     \\ \hline
\end{tabular}\label{tab:PALNet_with_4_loss}
% \vspace{-2mm}
\end{table}





==> ICAR2020_PALNet/tabs/AS_Accuracy_Different_Loss-SSCNet.tex <==
\begin{table}[tb]
\caption{Results of SSCNet trained with PA-Loss and Weighted Cross-Entropy Loss (WCE Loss). With SSCNet* denotes our implementation of SSCNet~\cite{song2017_SSCNet}.
}
% \vspace{-1mm}
\centering
\scalebox{1.0}
{
\begin{tabular}{l|l|lll|l}
\hline
Methods & Loss function & Precision         & Recall            & IoU               & mIoU              \\ \hline
SSCNet  & WCE Loss          & 75.4              & {\bfseries 96.3}  & 73.2              & 40.0              \\
SSCNet* & WCE Loss          & 76.5              & 95.7              & 74.8              & 42.1              \\
SSCNet* & PA-Loss            & {\bfseries 81.6}  & 91.6              & {\bfseries 76.0} & {\bfseries 43.4}   \\ \hline
\end{tabular}
\label{tab:loss-SSCNet}
}
% \vspace{-2mm}
\end{table}



==> ICAR2020_PALNet/tabs/NYU.tex <==
\begin{table*}[ht]
\caption{Results of various methods on NYU dataset~\cite{silberman2012NYUdataset}. Bold numbers represent the best score.}
% \vspace{-1mm}
\centering
{\begin{tabular}
{l |c c c|c c c c c c c c c c c c} 
\hline
& \multicolumn{3}{c|}{scene completion} & \multicolumn{12}{c}{semantic scene completion} \\ \hline
Method  & prec. & recall & IoU & \cellcolor{rgb1}ceil. & \cellcolor{rgb2}floor & \cellcolor{rgb3}wall & \cellcolor{rgb4}win. & \cellcolor{rgb5}chair & \cellcolor{rgb6}bed & \cellcolor{rgb7}sofa & \cellcolor{rgb8}table & \cellcolor{rgb9}tvs & \cellcolor{rgb10}furn. & \cellcolor{rgb11}objs. & mIoU \\ 
\hline
Lin et al.~\cite{lin2013holistic}   & 58.5 & 49.9 & 36.4 &  0.0 & 11.7 & 13.3 & {\bfseries 14.1} &  9.4 & 29.0 & 24.0 &  6.0 &  7.0 & 16.2 &  1.1 & 12.0\\ %& 2013NYU
Geiger et al.~\cite{geiger2015joint} & 65.7 & 58.0 & 44.4 & 10.2 & 62.5 & 19.1 &  5.8 &  8.5 & 40.6 & 27.7 &  7.0 &  6.0 & 22.6 &  5.9 & 19.6\\ %&2015NYU
    \hline
SSCnet~\cite{song2017_SSCNet} & 59.3 & {\bfseries 92.9} & 56.6 & 15.1 & 94.6 & 24.7 & 10.8 & 17.3 & 53.2 & 45.9 & 15.9 & 13.9 & 31.1 & 12.6 & 30.5\\ %2017
TS3D~\cite{Garbade2018_twoStream}     & 64.9 & 88.8 & 60.2 & 8.2 & 94.1 & 26.4 & 19.2 & 17.2 & 55.5 & 48.4 & 16.4 & 22.0 & 34.0 & {\bfseries 17.1} & 32.6\\   % v2
EsscNet~\cite{zhang2018efficient}   & {\bfseries 71.9} & 71.9 & 56.2 & 17.5 & 75.4 & 25.8 &  6.7 & 15.3 & 53.8 & 42.4 & 11.2 &    0 & 33.4 & 11.8 & 26.7\\ 
DDR-SSC~\cite{li2019rgbd}  & 71.5  & 80.8 & 61.0 & 21.1 & 92.2 & {\bfseries 33.5} & 6.8 & 14.8 & 48.3 & 42.3 & 13.2 &  13.9 & 35.3 & 13.2 & 30.4 \\ 
VVNet~\cite{guo2018_VVNet}  & 69.8 & 83.1 & 61.1 & 19.3 & {\bfseries 94.8} & 28.0 & 12.2 & 19.6 & {\bfseries 57.0} & {\bfseries 50.5} & {\bfseries 17.6} & 11.9 & 35.6 & 15.3 & 32.9\\ 
\hline
PALNet(ours)      &  68.7 & 85.0 & {\bfseries 61.3} & {\bfseries 23.5} & 92.0 & 33.0 & 11.6 & {\bfseries 20.1} & 53.9 & 48.1 & 16.2 & {\bfseries 24.2} & {\bfseries 37.8} & 14.7 & {\bfseries 34.1}\\ 
\hline
\end{tabular}\label{tab:results_on_nyu}}
\end{table*}


==> ICAR2020_PALNet/tabs/NYUCAD.tex <==
\begin{table*}[ht]
\caption{
Results of various methods on NYUCAD dataset~\cite{firman2016NYUCAD}. Bold numbers represent the best score.
}
% \vspace{-1mm}
\centering
\scalebox{1.0}
{\begin{tabular}
{l |c c c|c c c c c c c c c c c c}  
\hline
& \multicolumn{3}{c|}{scene completion} & \multicolumn{12}{c}{semantic scene completion} \\ \hline
Method  & prec. & recall & IoU & \cellcolor{rgb1}ceil. & \cellcolor{rgb2}floor & \cellcolor{rgb3}wall & \cellcolor{rgb4}win. & \cellcolor{rgb5}chair & \cellcolor{rgb6}bed & \cellcolor{rgb7}sofa & \cellcolor{rgb8}table & \cellcolor{rgb9}tvs & \cellcolor{rgb10}furn. & \cellcolor{rgb11}objs. & mIoU \\ 
\hline
Zheng et al.~\cite{zheng2013beyond}    & 60.1 & 46.7 & 34.6 & - & - & - & - & - & - & - & - & - & - & - & - \\
Firman et al.~\cite{firman2016NYUCAD}  & 66.5 & 69.7 & 50.8 & - & - & - & - & - & - & - & - & - & - & - & - \\
\hline
%   SSCnet        & 75.0 & 92.3 & 70.3 & - \\   % trained on NYUCAD
SSCnet~\cite{song2017_SSCNet}    & 75.4 & {\bfseries96.3} & 73.2  & 32.5 & 92.6 & 49.2 &  8.9 & 33.9 & 57.0 & 59.5 & 28.3 &  8.1 & 44.8 & 25.1 & 40.0 \\   % trained on SUNCG and NYUCAD
TS3D~\cite{Garbade2018_twoStream}& 80.2 & 94.4 & 76.5  & 34.4 & {\bfseries93.6} & 47.7 & {\bfseries31.8} & 32.2 & {\bfseries65.2} & 54.2 & 30.7 & {\bfseries32.5} & {\bfseries50.1} & 30.7 & 45.7 \\  
DDR-SSC~\cite{li2019rgbd}   & {\bfseries 88.7} & 88.5 & 79.4 & 54.1 & 91.5 & 56.4 & 14.9 & 37.0 & 55.7 & 51.0 &  28.8 & 9.2 & 44.1 &  27.8 & 42.8 \\
VVNet~\cite{guo2018_VVNet}      & 86.4 & 92.0 & 80.3   & - & - & - & - & - & - & - & - & - & - & - & - \\ 
\hline
PALNet    & 87.2 & 91.7 & {\bfseries80.8}   & {\bfseries54.8} & 92.8 & {\bfseries60.3} & 15.3 & {\bfseries43.1} & 60.7 & {\bfseries59.9} & {\bfseries37.6} &  8.1 & 48.6 & {\bfseries31.7} & {\bfseries46.6} \\
\hline
\end{tabular}\label{tab:results_on_nyucad}}
\end{table*}


==> ICAR2020_PALNet/tabs/Params.tex <==
% \vspace{-0.3cm}
\begin{table}[!tb]
\caption{
The number of parameters, inference speed and GPU memory usage of SSCNet~\cite{song2017_SSCNet}
% , DDR-SSC~\cite{li2019rgbd} 
and the proposed PALNet.
}
% \vspace{-2mm}
\begin{center}
\scalebox{0.95}
{
\begin{tabular} {l|c|c|c|c|c|c} 
\hline
\multicolumn{1}{c|}{Method} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Params\\ (k)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}FLOPs\\ (G)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Speed\\ (FPS)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Memory\\ (M)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Network \\ Depth\end{tabular}} &
\multicolumn{1}{c}{\begin{tabular}[c]{@{}c@{}}SSC\\ IoU(\%)\end{tabular}}         \\  \hline
SSCNet 	& 930.0             & 163.8         & 0.7          & 5305            &    14       & 40.0          \\
% DDR-SSC        & \textbf{195.0}    & \textbf{27.2} & \textbf{1.5} & \textbf{1829} & \textbf{44}    & 30.4          \\
% PALNet        & 223.0             & 78.8          & 1.2  & 3717  & 25  & \textbf{46.6}          \\
PALNet        & \textbf{223.0}             & \textbf{78.8}          & \textbf{1.2}  & \textbf{3717}  & \textbf{25}  & \textbf{46.6}          \\
\hline
\end{tabular}
}
\label{tab:SpeedMemory}
\end{center}
% \vspace{-2mm}
\end{table}
% \vspace{-0.6cm}

==> ICAR2020_PALNet/tabs/TwoBranches.tex <==
\begin{table*}[htbp]
\caption{
% Ablation study for the hybrid structure. Results are tested on the NYUCAD dataset~\cite{firman2016NYUCAD}.
Results of variant PALNets and SSCNet~\cite{song2017_SSCNet}.
}
% \vspace{-2mm}
\centering
\scalebox{1.0}
{\begin{tabular}
{l |c c c|c c c c c c c c c c c c}  
\hline
& \multicolumn{3}{c|}{scene completion} & \multicolumn{12}{c}{semantic scene completion} \\ \hline
Method  & prec. & recall & IoU & \cellcolor{rgb1}ceil. & \cellcolor{rgb2}floor & \cellcolor{rgb3}wall & \cellcolor{rgb4}win. & \cellcolor{rgb5}chair & \cellcolor{rgb6}bed & \cellcolor{rgb7}sofa & \cellcolor{rgb8}table & \cellcolor{rgb9}tvs & \cellcolor{rgb10}furn. & \cellcolor{rgb11}objs. & avg. \\ 
\hline

SSCnet~\cite{song2017_SSCNet}    & 75.4 & {\bfseries96.3} & 73.2  & 32.5 & 92.6 & 49.2 &  8.9 & 33.9 & 57.0 & 59.5 & 28.3 &  8.1 & 44.8 & 25.1 & 40.0 \\   % trained on SUNCG and NYUCAD
PALNet-3D                     & 83.3 & 94.5 & 79.1   & 49.1 & 92.3 & 56.2 &  6.8 & 36.6 & {\bfseries62.5} & 57.6 & 34.6 &  5.9 & 45.6 & 30.7 & 43.5 \\ 
PALNet-2D                     & 83.5 & 93.4 & 78.8   & 52.2 & 92.0 & 56.6 & {\bfseries20.1} & 40.2 & 61.1 & 58.8 & 33.9 & {\bfseries17.1} & 45.3 & 30.0 & 46.1 \\ 
PALNet-hybrid    & {\bfseries87.2} & 91.7 & {\bfseries80.8}   & {\bfseries54.8} & {\bfseries92.8} & {\bfseries60.3} & 15.3 & {\bfseries43.1} & 60.7 & {\bfseries59.9} & {\bfseries37.6} &  8.1 & {\bfseries48.6} & {\bfseries31.7} & {\bfseries46.6} \\
\hline
\end{tabular}\label{tab:results_2barnch}}
% \vspace{-2mm}
\end{table*}
